GIT: A Generative Image-to-text Transformer for Vision and Language

In this paper, we design and train a Generative Image-to-text Transformer, GIT, to unify vision-language tasks such as image/video captioning and question answering. While generative models provide a consistent network architecture between pre-training and fine-tuning, existing work typically contains complex structures (uni/multi-modal encoder/decoder) and depends on external modules such as object detectors/taggers and optical character recognition (OCR). In GIT, we simplify the architecture as one image encoder and one text decoder under a single language modeling task. We also scale up the pre-training data and the model size to boost the model performance. Without bells and whistles, our GIT establishes new state of the arts on 12 challenging benchmarks with a large margin. For instance, our model surpasses the human performance for the first time on TextCaps (138.2 vs. 125.5 in CIDEr). Furthermore, we present a new scheme of generation-based image classification and scene text recognition, achieving decent performance on standard benchmarks. Codes are released at \url{https://github.com/microsoft/GenerativeImage2Text}.

==> ack.tex <==

\section*{Acknowledgement}
We would like to thank 
Lin Liang for her help on scene text recognition experiments,
Houdong Hu and Min Gao for their help on the pre-training data, and
Lu Yuan and Bin Xiao for their help on the pre-trained image encoder. We would like to thank 
Nguyen Bach, Jiayuan Huang, Luis Vargas, Yumao Lu, Michael Zeng, and Xuedong Huang  for their support.

==> checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Supplementary materials shows all the hyper-parameters for reproducing the results.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In experiment settings and supplementary materials}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{large-scale training is costly}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In supplementary materials}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In supplementary materials}
  \item Did you mention the license of the assets?
    \answerYes{In supplementary materials}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> fig/TaxImageNet2012GenV1_vis_outlier.tex <==
\begin{figure}[th!]
\centering
\small
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}}
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00023430.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00020643.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00046563.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00045848.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00017781.JPEG.jpg}\\
{\textbf{Pred}}: four - poster & {\textbf{Pred}}: four - poster & {\textbf{Pred}}: ping - pong ball & {\textbf{Pred}}: long - horned beetle & {\textbf{Pred}}: three - toed sloth\\
\textbf{GT}: four-poster & \textbf{GT}: four-poster & \textbf{GT}: ping-pong ball & \textbf{GT}: long-horned beetle & \textbf{GT}: three-toed sloth\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00044966.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00019003.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00011554.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00043321.JPEG.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxImageNet2012GenV1/outlier/ILSVRC2012_val_00019328.JPEG.jpg}\\
{\textbf{Pred}}: sulphur - crested cockatoo & {\textbf{Pred}}: four - poster & {\textbf{Pred}}: sulphur - crested cockatoo & {\textbf{Pred}}: jack - o'- lantern & {\textbf{Pred}}: sulphur - crested cockatoo\\
\textbf{GT}: sulphur-crested cockatoo & \textbf{GT}: four-poster & \textbf{GT}: sulphur-crested cockatoo & \textbf{GT}: jack-o'-lantern & \textbf{GT}: sulphur-crested cockatoo\\
\end{tabular}
\caption{Image samples on which the prediction of our GIT is out of the 1K categories on ImageNet-1K.}
\label{fig:outlier}
\end{figure}

==> fig/TaxVizWizVQA_vis_random.tex <==
\begin{table}
\centering
\small
\caption{Visualization of random samples for the validation set on VizWiz-VQA. Red/blue: correct or wrong of the prediction.}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}}
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/1372.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/3807.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/402.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/3013.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/2401.jpg}\\
\textbf{Q}: What is this? & \textbf{Q}: What is this? & \textbf{Q}: Is this valium? & \textbf{Q}: What color is this? & \textbf{Q}: What is in this tin?\\
{\color{red}\textbf{iVLM}}: unanswerable & {\color{red}\textbf{iVLM}}: calculator & {\color{red}\textbf{iVLM}}: unanswerable & {\color{red}\textbf{iVLM}}: grey & {\color{red}\textbf{iVLM}}: corn\\
\textbf{GT}: unsuitable, fabric, this grand, unanswerable & \textbf{GT}: keypad, scientific calculator, calculator, speaking calculator & \textbf{GT}: no, unsuitable image, unanswerable, unable to read medication name & \textbf{GT}: blue, grey, black, black color & \textbf{GT}: unanswerable, unsuitable, cream corn, this back but looks like could be corn, corn\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/1124.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/4154.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/2669.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/3561.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/1947.jpg}\\
\textbf{Q}: Who is this picture? & \textbf{Q}: What is this question? & \textbf{Q}: What does my screen say? & \textbf{Q}: What kind of can food is this? & \textbf{Q}: What is the title of the book?\\
{\color{red}\textbf{iVLM}}: unanswerable & {\color{blue}\textbf{iVLM}}: cleaning brush & {\color{red}\textbf{iVLM}}: unsuitable & {\color{blue}\textbf{iVLM}}: unsuitable & {\color{blue}\textbf{iVLM}}: unanswerable\\
\textbf{GT}: crowd, unanswerable, crowd people, computer screen, people at event, no 1, laptop screen & \textbf{GT}: unanswerable, dish cleaner, pipe cleaner, i dont know, lint brush, brush, bottle cleaner & \textbf{GT}: unanswerable, i cant tell, unsuitable, too far away to read, i cant tell what says & \textbf{GT}: vegetables, salmon, unanswerable, bamboo shoots, noodles, soup, baby corn & \textbf{GT}: auf die lange kommt es, auf die lange, auf die länge kommt es\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/2687.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/4090.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/1532.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/230.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxVizWizVQA/random/712.jpg}\\
\textbf{Q}: Could you tell me what brand this is? Thank you. & \textbf{Q}: Is the label showing? And what is in this bottle? & \textbf{Q}: Who is the fifth president and who is on the six dollar bill? & \textbf{Q}: Can you tell what brand and model this television is, please? Thank you. & \textbf{Q}: How many calories are in Insure? Are you holding it down? Oh no. Am I supposed to hold it down? No, you just hit. I hit it once and then I talked. And then you hit it again when you're done.\\
{\color{red}\textbf{iVLM}}: grace & {\color{red}\textbf{iVLM}}: unanswerable & {\color{red}\textbf{iVLM}}: abraham lincoln & {\color{blue}\textbf{iVLM}}: unsuitable & {\color{blue}\textbf{iVLM}}: \\
\textbf{GT}: grace, grace hot pepper sauce & \textbf{GT}: unanswerable, unsuitable, nutrition facts for some type supplement, no, supplement facts visible only, yes diet supplements & \textbf{GT}: abe lincoln, lincoln, unanswerable, lincoln 0, abraham lincoln, james monroe no 6 dollar bill & \textbf{GT}: no, unsuitable image, unanswerable & \textbf{GT}: unsuitable image, dont know, unanswerable\\
\end{tabular}
\end{table}

==> fig/stvqa_vis_random.tex <==
\begin{table}
\centering
\small
\caption{Visualization on ST-VQA. Images are randomly sampled from the validation set. Red/blue: correct or wrong of the prediction.}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}@{~~}p{\fivewidth\linewidth}}
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/6.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/19.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/5.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/14.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/17.jpg}\\
\textbf{Q}: What letter is above the store on the right? & \textbf{Q}: What color is the traffic light? & \textbf{Q}: What is the numbers on the top sign? & \textbf{Q}: what year was the picture taken? & \textbf{Q}: What is the top street name?\\
{\color{red}\textbf{iVLM}}: t & {\color{red}\textbf{iVLM}}: red & {\color{blue}\textbf{iVLM}}: 2600 & {\color{red}\textbf{iVLM}}: 2011 & {\color{red}\textbf{iVLM}}: pitt\\
\textbf{GT}: t & \textbf{GT}: red & \textbf{GT}: 2563 & \textbf{GT}: 2011 & \textbf{GT}: pitt\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/10.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/0.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/4.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/1.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/9.jpg}\\
\textbf{Q}: What is the brand that is printed on the yellow sign behind the cameramen? & \textbf{Q}: What restaurant can you get this sandwich from? & \textbf{Q}: Which one is the "JAZZ" radio station? & \textbf{Q}: What is the time on the clock on top of the car? & \textbf{Q}: What is the name of the airline?\\
{\color{red}\textbf{iVLM}}: nikon & {\color{red}\textbf{iVLM}}: subway & {\color{blue}\textbf{iVLM}}: 92. 5 & {\color{blue}\textbf{iVLM}}: 2 : 00 & {\color{red}\textbf{iVLM}}: westjet\\
\textbf{GT}: nikon & \textbf{GT}: subway & \textbf{GT}: 93.3fm & \textbf{GT}: 2:03:00 & \textbf{GT}: westjet\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/12.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/7.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/11.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/15.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/3.jpg}\\
\textbf{Q}: What is the restaurant name? & \textbf{Q}: What is the brand of the liquor? & \textbf{Q}: What kind of car part are these items? & \textbf{Q}: What kind of business is on the black advertisment? & \textbf{Q}: who is the auther of the book ?\\
{\color{blue}\textbf{iVLM}}: felfa & {\color{red}\textbf{iVLM}}: araucana & {\color{red}\textbf{iVLM}}: oil filter & {\color{blue}\textbf{iVLM}}: dunpav & {\color{red}\textbf{iVLM}}: william gibson\\
\textbf{GT}: felfela & \textbf{GT}: araucana & \textbf{GT}: oil filter & \textbf{GT}: entertainment & \textbf{GT}: william gibson\\
\includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/2.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/18.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/16.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/13.jpg} & \includegraphics[width=1\linewidth,height=1\linewidth]{fig/image/TaxSTVQA/random/8.jpg}\\
\textbf{Q}: What text is displayed on the bottom right? & \textbf{Q}: What is the website listed? & \textbf{Q}: What is the full name of the street? & \textbf{Q}: What does this Churreria sell? & \textbf{Q}: Who took the photo and has a credit on it?\\
{\color{blue}\textbf{iVLM}}: estrelaa paulinho & {\color{blue}\textbf{iVLM}}: downtowntraveler. com & {\color{blue}\textbf{iVLM}}: prime box street & {\color{blue}\textbf{iVLM}}: chocolates & {\color{red}\textbf{iVLM}}: david baker\\
\textbf{GT}: estrelaaa paulinha & \textbf{GT}: downtowntraveler.com & \textbf{GT}: prime gilt box street & \textbf{GT}: crepes and chocolates, crepes chocolates porr & \textbf{GT}: david baker, photo by: david baker baker david @gmail.com\\
\end{tabular}
\end{table}
